P^3 Ranker: Mitigating the Gaps between Pre-training and Ranking Fine-tuning with Prompt-based Learning and Pre-finetuning

Compared to other language tasks, applying pre-trained language models (PLMs) for search ranking often requires more nuances and training signals. In this paper, we identify and study the two mismatches between pre-training and ranking fine-tuning: the training schema gap regarding the differences in training objectives and model architectures, and the task knowledge gap considering the discrepancy between the knowledge needed in ranking and that learned during pre-training. To mitigate these gaps, we propose Pre-trained, Prompt-learned and Pre-finetuned Neural Ranker (P^3 Ranker). P^3 Ranker leverages prompt-based learning to convert the ranking task into a pre-training like schema and uses pre-finetuning to initialize the model on intermediate supervised tasks. Experiments on MS MARCO and Robust04 show the superior performances of P^3 Ranker in few-shot ranking. Analyses reveal that P^3 Ranker is able to better accustom to the ranking task through prompt-based learning and retrieve necessary ranking-oriented knowledge gleaned in pre-finetuning, resulting in data-efficient PLM adaptation. Our code is available at https://github.com/NEUIR/P3Ranker.

==> Figures/compare-all-senario.tex <==
\begin{figure}[h]
    \centering
    %\includegraphics[width=\linewidth]{Figures/task-pretrain.pdf}
    \includegraphics[width=\linewidth]{Figures/all-senario.pdf}
    \caption{Comparison in prompt-tuning.
    \label{fig:Comparison in prompt-tuning}}
\end{figure}




==> Tables/fullset_details.tex <==
\begin{table}
  \caption{Data statistics of Robust04 and MS MARCO.}
  \label{tab:statistic}
  \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|r|rr} 
    \hline
    \multirow{2}{*}{\textbf{Statistics}}        & \textbf{Robust04}     & \multicolumn{2}{c}{\textbf{MS MARCO}}  \\
                                                & \textbf{Test}         & \textbf{Train}    & \textbf{Dev}       \\ 
    \hline
    \# Queries                                  &                       &                  530k & 6980          \\
    \# Avg. Relevance Annotations per q         &                       &                   1&  1         \\
    \hline
    \# Documents                                &                       & \multicolumn{2}{c}{8.8M}  \\
    \hline
    \end{tabular}
   }
\end{table}

==> Tables/overall-rb04.tex <==
\begin{table}
    \centering
    \small
    

    % \begin{tabular}{l | p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.0cm}<{\raggedleft}| p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.0cm}<{\raggedleft}} 
    \resizebox{\linewidth}{!}{
     \begin{tabular}{l|l|l|l|l} 
    \hline
    \textbf{Method} & \textbf{0.2\%} & \textbf{2\%} & \textbf{20\%} & \textbf{100\%}  \\ 
    \hline
    \multicolumn{5}{l}{\textbf{Vanilla Fine-tuning}} \\
    \hline
    BERT-large &  &  &  &  \\
    RoBERTa-large &  &  &  &  \\
    \hline
    \multicolumn{5}{l}{\textbf{Prompt-based Method}} \\
    \hline
    RoBERTa-large &  &  &  &  \\
    T5-large &  &  &  &  \\
    \hline
    \end{tabular} }
    \caption{Overall results on Robust04.}
    \label{tab:overall-results-rb04}
\end{table}

==> Tables/pretrain_task.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{rrrrrr}
    \hline
    Task& Label& \multicolumn{1}{c}{Input text}& Output text &\multicolumn{2}{c}{Symbol meaning}\\
    \hline
    \multirow{3}{*}{MNLI}& 0& \multirow{3}{*}{
    mnli hypothesis: <h> precise:<p> entailment: }& true &<h>&hypothesis  \\
    \multirow{3}{*}{}& 1& \multirow{3}{*}{}& neutral&<p>&premise\\
    \multirow{3}{*}{}& 2& \multirow{3}{*}{}& false&-&-\\
    \hline
    \multirow{2}{*}{NQ}& 0& \multirow{2}{*}{
    NQ questions: <q> document:<d> answered: }& false&<q>&question   \\
    \multirow{2}{*}{}& 1& \multirow{2}{*}{}& true&<d>&document\\
    \hline
    \end{tabular}
    \caption{Pretrain Settings.}
    \label{tab:Pretrain Settings}
\end{table*}


==> Tables/subset_details.tex <==

\begin{table}
\small
\begin{tabular}{ r|r|r|r|r  }
 \hline
%  \multicolumn{5}{c}{MS MARCO} \\
%  \hline
 \multicolumn{3}{c|}{Train }& \multicolumn{2}{c}{Dev} \\
 \hline            
    q   & (q,d+)    & (q,d-)    & q     & (q,d) \\
  \hline
    530k& 530k      & 530k      & 500   & 500k  \\
    1k  & 1k        & 1k        & 500   & 500k \\
    50  & 50        & 50        & 50    & 50k \\
    5   & 5         & 5         & 5     & 5k\\
 \hline
\end{tabular}
\caption{Dataset statistics of our processed MS MARCO.}
\label{tab:data partition details}
\end{table}

==> Tables/t5.tex <==
\begin{table*}[t]
    \centering
    \small
    

    % \begin{tabular}{l | p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.0cm}<{\raggedleft}| p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.0cm}<{\raggedleft}} 
    \resizebox{\linewidth}{!}{
     \begin{tabular}{l|ll|ll|ll|ll} 
    \hline
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{5}} & \multicolumn{2}{c|}{\textbf{50}} & \multicolumn{2}{c|}{\textbf{1k}} & \multicolumn{2}{c}{\textbf{530k}}  \\ 
    \cline{2-9}
        & \textbf{MRR@10} & \textbf{R@10} & \textbf{MRR@10} & \textbf{R@10} & \textbf{MRR@10} & \textbf{R@10} & \textbf{MRR@10} & \textbf{R@10} \\
    \hline
    \textbf{T5-large} & 0.1186& 0.2882& 0.2250& 0.4622& 0.2743& 0.5372& 0.3819&0.6535 \\
    w/o Multi-task Supervised Training & 0.0029&0.0112 & 0.1117&0.0043 & 0.1616&0.3559 & 0.3496&0.6268 \\
    w/o Prompt & 0.0036&0.0118& 0.0234&0.0722 & 0.1559&0.3691 & 0.3638&0.6373 \\
    \hline
    \end{tabular} }
    \caption{T5 ablation study.}
    \label{tab:prompt-t5}

\end{table*}
